An implicit large-eddy simulation perspective on the flow over periodic hills

The periodic hills simulation case is a well-established benchmark for computational fluid dynamics solvers due to its complex features derived from the separation of a turbulent flow from a curved surface. We study the case with the open-source implicit large-eddy simulation (ILES) software Lethe. Lethe solves the incompressible Navier-Stokes equations by applying a stabilised continuous finite element discretisation. The results are validated by comparison to experimental and computational data available in the literature for Re = 5600. We study the effect of the time step, averaging time, and global mesh refinement. The ILES approach shows good accuracy for average velocities and Reynolds stresses using less degrees of freedom than the reference numerical solution. The time step has a greater effect on the accuracy when using coarser meshes, while for fine meshes the results are rapidly time-step independent when using an implicit time-stepping approach. A good prediction of the reattachment point is obtained with several meshes and this value approaches the experimental benchmark value as the mesh is refined. We also run simulations at Reynolds equal to 10600 and 37000 and observe promising results for the ILES approach.

==> src/nomenclature.tex <==
% Create nomenclature

\nomenclature[S]{$L_x$}{Length of geometry in the x direction \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$L_y$}{Length of geometry in the y direction \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$L_z$}{Length of geometry in the z direction \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$h$}{Height of a hill \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$u_B$}{Bulk velocity \nomunit{$\SI{}{\metre \per \second}$}}
\nomenclature[S]{$\nu$}{Kinematic viscosity \nomunit{$\SI{}{\metre \squared \per \second}$}}
\nomenclature[S]{$\bm{u}$}{Velocity vector \nomunit{$\SI{}{\metre \per \second}$}}
\nomenclature[S]{$\bm{u}_h$}{Approximate solution of the velocity vector \nomunit{$\SI{}{\metre \per \second}$}}
\nomenclature[S]{$\Omega$}{Domain of the finite element space \nomunit{-}}
\nomenclature[S]{$\Gamma$}{Boundary of the finite element space \nomunit{-}}
\nomenclature[S]{$\Omega^e$}{Domain of a finite element \nomunit{-}}
\nomenclature[S]{$\Gamma^e$}{Boundary of a finite element \nomunit{-}}
\nomenclature[S]{$p$}{Pressure \nomunit{Pa}}
\nomenclature[S]{$p*_h$}{Approximate solution of the pressure over the density \nomunit{Pa}}
\nomenclature[S]{$\rho$}{Density \nomunit{$\SI{}{\kilo \gram \per \metre \cubed}$}}
\nomenclature[S]{$\bm{\tau}$}{Deviatoric stress tensor}
\nomenclature[S]{$\bm{f}$}{Body force \nomunit{N}}
\nomenclature[S]{$\alpha$}{Elongation of geometry in x direction \nomunit{-}}
\nomenclature[S]{$\eta$}{Kolmogorov length scale \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$\beta$}{Momentum source term for pressure driven flow \nomunit{$\SI{}{\kilo \gram \per \metre \squared \per \second \squared}$}}
\nomenclature[S]{$\epsilon$}{Dissipation tensor \nomunit{$\SI{}{\metre \squared \per \second \cubed}$}}
\nomenclature[S]{$L$}{Length-scale of largest eddy present in the flow \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$y^+$}{Dimensionless distance from the lower wall \nomunit{-}}
\nomenclature[S]{$y_{cc}$}{Half distance from wall to wall-nearest grid point \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$y(x)$}{Elevation of bottom wall \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$u_{\tau}$}{Friction velocity \nomunit{$\SI{}{\metre \per \second}$}}
\nomenclature[S]{$\tau_w$}{Wall shear stress \nomunit{$\SI{}{\kilo \gram \per \metre \per \second \squared}$}}
\nomenclature[S]{$\Delta x^+$}{Dimensionless cell width in the x direction \nomunit{-}}
\nomenclature[S]{$\Delta z^+$}{Dimensionless cell width in the z direction \nomunit{-}}
\nomenclature[S]{$\Delta x$}{Cell width in the x direction \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$\Delta z$}{Cell width in the z direction \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$\Delta y$}{Cell width in the y direction \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$\Delta$}{Cell size \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$u$}{Average velocity in the x direction \nomunit{$\SI{}{\metre \per \second}$}}
\nomenclature[S]{$v$}{Average velocity in the y direction \nomunit{$\SI{}{\metre \per \second}$}}
\nomenclature[S]{$u'u'$}{Reynolds normal stress in the x direction \nomunit{$\SI{}{\metre \squared \per \second \squared}$}}
\nomenclature[S]{$v'v'$}{Reynolds normal stress in the y direction \nomunit{$\SI{}{\metre \squared \per \second \squared}$}}
\nomenclature[S]{$w'w'$}{Reynolds normal stress in the z direction \nomunit{$\SI{}{\metre \squared \per \second \squared}$}}
\nomenclature[S]{$u'v'$}{Reynolds shear stress on the y plane in the x direction \nomunit{$\SI{}{\metre \squared \per \second \squared}$}}
\nomenclature[S]{t}{Time step \nomunit{$\SI{}{\second}$}}
\nomenclature[S]{$\xi$}{Compression ratio \nomunit{-}}
\nomenclature[S]{$N_f$}{Number of grid points on the fixed (coarsest) mesh \nomunit{-}}
\nomenclature[S]{$N_a$}{Final number of grid points on the adaptive mesh \nomunit{-}}
\nomenclature[S]{$Re$}{Reynolds number \nomunit{-}}
\nomenclature[S]{$q$}{Weight function for pressure \nomunit{-}}
\nomenclature[S]{$\bm{v}$}{Weight function for velocity \nomunit{-}}
\nomenclature[S]{$\bm{\psi}$}{Shape function for velocity \nomunit{-}}
\nomenclature[S]{$\bm{\phi}$}{Shape function for pressure \nomunit{-}}
\nomenclature[S]{$h_{conv}$}{Size of the element related to convective transport \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$h_{diff}$}{Size of the element related to diffusion \nomunit{$\SI{}{\metre}$}}
\nomenclature[S]{$R$}{Residual \nomunit{-}}
\nomenclature[S]{$e$}{Error in reattachment point at a given number of flow through times \nomunit{-}}
\nomenclature[S]{$c$}{Manually defined constant for averaging error \nomunit{-}}
\nomenclature[S]{$T-f$}{Number of flow through times \nomunit{-}}

\nomenclature[A]{CFD}{Computational fluid dynamics}
\nomenclature[A]{CFL}{Courant–Friedrichs–Lewy (condition)}
\nomenclature[A]{RANS}{Reynolds averaged Navier-Stokes}
\nomenclature[A]{LES}{Large eddy simulation}
\nomenclature[A]{DES}{Detached eddy simulation}
\nomenclature[A]{DNS}{Direct numerical simulation}
\nomenclature[A]{FD}{Finite difference (method)}
\nomenclature[A]{FEM}{Finite element method}
\nomenclature[A]{FVM}{Finite volume method}
\nomenclature[A]{SGS}{Sub-grid scale}
\nomenclature[A]{AMR}{Adaptive mesh refinement}
\nomenclature[A]{GLS}{Galerkin least-squares}
\nomenclature[A]{MPI}{Message passing interface}
\nomenclature[A]{PDE}{Partial differential equation}
\nomenclature[A]{RHS}{Right hand side (of an equation)}
\nomenclature[A]{LHS}{Left hand side (of an equation)}
\nomenclature[A]{GMRES}{Generalised minimal residual method}
\nomenclature[A]{ILU}{Incomplete lower-upper (preconditioner)}
\nomenclature[A]{BDF2}{$2^{nd}$ order backward difference}
\nomenclature[A]{PIV}{Particle image velocimetry}
\nomenclature[A]{LDA}{Laser doppler anemometry}
